Mirror: A Multiple-perspective Self-Reflection Method for Knowledge-rich Reasoning

While Large language models (LLMs) have the capability to iteratively reflect on their own outputs, recent studies have observed their struggles with knowledge-rich problems without access to external resources. In addition to the inefficiency of LLMs in self-assessment, we also observe that LLMs struggle to revisit their predictions despite receiving explicit negative feedback. Therefore, We propose Mirror, a Multiple-perspective self-reflection method for knowledge-rich reasoning, to avoid getting stuck at a particular reflection iteration. Mirror enables LLMs to reflect from multiple-perspective clues, achieved through a heuristic interaction between a Navigator and a Reasoner. It guides agents toward diverse yet plausibly reliable reasoning trajectory without access to ground truth by encouraging (1) diversity of directions generated by Navigator and (2) agreement among strategically induced perturbations in responses generated by the Reasoner. The experiments on five reasoning datasets demonstrate that Mirror's superiority over several contemporary self-reflection approaches. Additionally, the ablation study studies clearly indicate that our strategies alleviate the aforementioned challenges.

==> sections/representation.tex <==
\section{Discovering True/False via representation learning}
Although we can force the model to follow the instructions and change its initial prediction, large percentage of predictions are not changed across different context perturbation. Moreover, in practical setting, we actually do not have access to ground truth  as oracle critic to give accurate feedback. In this sense, we would like to explore if the model could check its True/False output in an unsupervised way. One popular way is to identify the activations when feeding the input, recent work has shown that the activations from True and False statements can be mapped into clearly separate spaces. Inspired by this, we 


\subsection{Out-of-Distribution Evaluation}




==> sections/widthfirst.tex <==
\section{Align with the instructions from Critic}


By comparing the 100-\#correct and \#changes for \textsl{Groundtruth}.  We find that there is a gap between "answer is incorrect" and the behaviour that the model will change its current prediction. This misalignment is commonly observed in LLMs, and lots of work focusing on how to align the  LLMs' behaviour to human instructions. Inspired by \textit{superficial alignment} in \citet{DBLP:journals/corr/abs-2305-11206} that a model’s capabilities are primarily gained during pre-training, while alignment is essentially to match a sub-distribution close to the instruction. Moreover, empirical studies shows that the fine-tuning on annotated instruction dataset can be omitted in order to achieve alignment. Our solutions stems from this parameter-frozen alignment, specially for the two categories, i.e, with prompts constraints~\cite{DBLP:journals/corr/abs-2310-14542} and decoding constraints for generation steering. 

\subsection{Prompt constraints for instruction alignment}
In our self-reflection settings, the LLMs are supposed to obey the instructions and conduct corresponding revision in the next round. Based on the observations that LLMs often fail to change their predictions given the reflection saying that "your previous trial was unsuccessful", we proposed three prompt constraints as part of the input fed to LLM and the results are shown in Table~\ref{tab:input_perturb}. \textsl{NegReflect} demonstrates the clear improvements across all the datasets and models, while the promotion on GPT3.5 is the 
minimal. This can be explained that larger model are more confident with its internal knowledge and less vulnerable to given noisy text. For tasks, the improvements over HotPotQA is less significant than MMLU, as HotpotQA solutions heavily relies on the given context which is longer than the prompt constraints. The three strategies have similar length, but the \textbf{NegReflect} is applied as a prefix for the generated reflection, that is, it is at the end of prompting. The success of \textsl{NegReflect} is also consistent with the findings in 


\subsubsection{Long context are robust to input perturbation}
\subsubsection{Larger model are robust to input perturbation}

\subsection{Steering  generation via constraints}
Beyond following the instruction to revise the last unsuccessful prediction, we need to make corresponding revisions according to the key elements in the feedback. Inspired by traditional conditional generation tasks which target at generating text with desirable attributes, we propose to generate response constrained by the key elements in the feedback. Specially, we firstly summarize the key phrases using LLMs, then 
a lexically constrained generation~\cite{DBLP:conf/nips/QinWKC22} is applied to the decoding phrase. 

